Fixing by Mixing: A Recipe for Optimal Byzantine ML under Heterogeneity

Byzantine machine learning (ML) aims to ensure the resilience of distributed learning algorithms to misbehaving (or Byzantine) machines. Although this problem received significant attention, prior works often assume the data held by the machines to be homogeneous, which is seldom true in practical settings. Data heterogeneity makes Byzantine ML considerably more challenging, since a Byzantine machine can hardly be distinguished from a non-Byzantine outlier. A few solutions have been proposed to tackle this issue, but these provide suboptimal probabilistic guarantees and fare poorly in practice. This paper closes the theoretical gap, achieving optimality and inducing good empirical results. In fact, we show how to automatically adapt existing solutions for (homogeneous) Byzantine ML to the heterogeneous setting through a powerful mechanism, we call nearest neighbor mixing (NNM), which boosts any standard robust distributed gradient descent variant to yield optimal Byzantine resilience under heterogeneity. We obtain similar guarantees (in expectation) by plugging NNM in the distributed stochastic heavy ball method, a practical substitute to distributed gradient descent. We obtain empirical results that significantly outperform state-of-the-art Byzantine ML solutions.

==> cenna-algorithm.tex <==
\section{Nearest Neighbor Mixing ($\cenna$)}

In this section, we introduce our robust primitive $\cenna$.
We propose $\cenna$ (nearest neighbor mixing), a pre-aggregation procedure designed to boost the precision of the aggregation operation. 
$\cenna$ takes input vectors $x_1,\ldots,x_n \in \R^d$ and replaces each vectors with the average of its $n-f$ nearest neighbors.
Formally, the vectors $(y_1, \ldots, y_n) = \cenna{(x_1,\ldots,x_n)}$ are obtained as follows:
\begin{equation*}
    y_j \coloneqq \frac{1}{n-f} \sum_{i \in \mathcal{N}_j} x_i,~ \forall j \in [n],
\end{equation*}
where $\mathcal{N}_j$ is the set of indices of the $n-f$ closest vectors to $x_j$ in $(x_1,\ldots,x_n)$, with respect to the Euclidean distance.
Intuitively, since for us the inputs will be (stochastic) gradients, $\cenna$ "mixes" the gradients thereby artificially allowing workers to compute gradients on the data of other workers, as illustrated in Figure~\ref{}.
The corresponding algorithm is summarized in Algorithm~\ref{algo:cenna}.

\begin{algorithm}[t!]
\label{algo:cenna}
\textbf{Input:} number of inputs $n$, number of malicious inputs $f < n$, vectors $x_1, \ldots, x_n \in \R^d$.

\For{$i = 1 \ldots n$}{
    Sort inputs w.r.t. distance to $x_i$:
    \begin{equation*}
        \|x^{(i)}_{1:n} - x_i\| \leq \ldots \leq \|x^{(i)}_{n:n} - x_i\|;
    \end{equation*}
    Average the $n-f$ nearest neighbors:
    \begin{equation*}
        y_i \gets \frac{1}{n-f} \sum_{j=1}^{n-f} x^{(i)}_{j:n};
    \end{equation*}
}

\textbf{return} $y_1, \ldots, y_n$\;
\caption{Nearest neighbor mixing ($\cenna$)}
\end{algorithm}

==> convergence.tex <==
\section{Convergence Analysis}

We now provide convergence guarantees for any $(f,\kappa)$-robust aggregation rule.

% \ysf{Here tight convergence analysis with diminishing stepsizes + momentum}

\begin{assumption}[Bounded variance]
\label{asp:bnd_var}
There exists a real value $\sigma < \infty$ such that for each worker $w_i$ and all $\theta{} \in \mathbb{R}^d$,
\begin{equation*}
    \mathbb{E}_{z \sim \mathcal{U}{(\D_i)}}{\left [
    \norm{ \nabla_{\theta{}}{\ell{(\theta,z)}} - \nabla \loss_i\left(\theta{}\right)}^2
    \right ]}
    \leq \sigma^2.
\end{equation*}
\end{assumption}

\begin{assumption}[Smoothness]
\label{asp:lip}
There exists a real value $L < \infty$ such that for each worker $w_i$ and all $\theta{}, \, \theta{}' \in \mathbb{R}^d$,
\begin{align*}
    \norm{\nabla \loss_{i}(\theta{}) - \nabla \loss_{i}(\theta{}')} \leq L \norm{\theta{} - \theta{}'}.
\end{align*}
\end{assumption}


We now state our Byzantine resilience result in Theorem~\ref{thm:conv}. Essentially, we analyze the convergence of Algorithm~\ref{algo} when up to $f$ workers are Byzantine, under assumptions~\ref{asp:bnd_var},~\ref{asp:lip}, and \ref{asp:hetero}. For readability, we introduce the following notations.
\begin{align*}
    &\loss^* \coloneqq \inf_{\weight{} \in \R^d} \loss_{\H}(\weight{}),
    \quad a_1 \coloneqq 36,\\
    &a_2 \coloneqq 6 \sqrt{\loss_{\H}(\weight{0}) - \loss^*},
    \quad a_3 \coloneqq 1728L,\\ &a_4 \coloneqq 288L,
    \quad \text{and} \quad a_5 \coloneqq 24L\, a_2^2.
\end{align*}

\boxwrap{
\begin{theorem}
\label{thm:conv-gd}
Suppose that assumptions~\ref{asp:lip} and ~\ref{asp:hetero} hold true. 
Consider Algorithm~\ref{gd} with learning rate $\gamma = \nicefrac{1}{24L}$.
If $F$ is $(f,\kappa)$-robust, then for all $T \geq 1$
$$
   \frac{1}{T} \sum_{t=0}^{T-1} \norm{\nabla \loss_{\H} \left(\weight{t} \right)}^2 \hspace{-2pt}
    \leq  a_1 (\kappa+1) \nicefrac{f}{n} G^2
    + \frac{a_5}{T}.
$$
\end{theorem}
}

\paragraph{Tight upper bound.}
\textcolor{red}{The convergence rates are tight for both Algorithm~\ref{sgd} and Algorithm~\ref{gd}.}
% A lower bound was shown previously~\cite{karimireddy2022byzantinerobust,collaborativeElMhamdi21} on the norm of the gradient of any optimization algorithm:
% \begin{equation*}
%     \expect{\norm{\nabla \loss_{\H} \left(\hat{\weight{}} \right)}^2} = \Omega{(\nicefrac{f}{n}\, G^2)}.
% \end{equation*}
% The upper bound shown in Theorem~\ref{thm:conv} achieves an asymptotic error of $\mathcal{O}{\left( \kappa\, G^2 \right)}$.
% Therefore, our convergence analysis is tight for any aggregation rule achieving $\kappa$ of the order of $\nicefrac{f}{n}$.
% As seen in Theorem~\ref{thm:reduce-aggregate}, this order of $\kappa$ whenever $\kappa \in \mathcal{O}{(1)}$ and $\eta$ is of the order of $\nicefrac{f}{n}$.
% As we shall see in Section~\ref{sec:design}, it is possible to design mixing strategies with a reduction factor $\eta$ of the order of $\nicefrac{f}{n}$.

\boxwrap{
\begin{corollary}
\label{cor:resilience}
Suppose that assumptions~\ref{asp:lip} and ~\ref{asp:hetero} hold true. 
Consider Algorithm~\ref{gd} with learning rate $\gamma = \nicefrac{1}{24L}$.
If $F$ is $(f,\kappa)$-robust, then Algorithm~\ref{gd} is $(f,\varepsilon)$-resilient with
$\varepsilon = \mathcal{O}{\left(\nicefrac{f}{n}(\kappa+1)G^2\right)}$.
\end{corollary}
}

\boxwrap{
\begin{theorem}
\label{thm:conv}
Suppose that assumptions~\ref{asp:bnd_var},~\ref{asp:lip}, and ~\ref{asp:hetero} hold true. 
Consider Algorithm~\ref{sgd} with learning rate $$\gamma= \min{\left\{\frac{1}{24L}, ~ \frac{a_2}{\overline{\sigma}\sqrt{T}}\right\}} ~ \text{ where}$$
% \label{eqn:step-size}
% \end{align*}
\noindent $\overline{\sigma}^2 \coloneqq  \big(a_3 \kappa + \frac{a_4}{n-f}\big) \sigma^2$,
and momentum parameter $\beta = \sqrt{1 - 24 \gamma L} $.
If $F$ is $(f,\kappa)$-robust, then for all $T \geq 1$
% for all $\vartheta \in (0, \, 1)$ and $\varrho \in (1, \, 2)$ the following holds true:
% \footnotesize
{\small
\begin{align*}
   \frac{1}{T} \sum_{t=0}^{T-1} \expect{\norm{\nabla \loss_{\H} \left(\weight{t} \right)}^2} \hspace{-2pt}
    \leq  a_1 \kappa^* G^2
    + \frac{a_2 \overline{\sigma}}{\sqrt{T}}
    + \frac{a_5}{T}
    + \frac{a_2 a_4 \sigma^2}{n \overline{\sigma} T^{\nicefrac{3}{2}}}, 
\end{align*}
}
where $\kappa^* \leq \nicefrac{f}{n} (\kappa + 1)$,
and the expectation is over the randomness of the data subsampling.
\end{theorem}
}




